Connectivity Maintenance for Multi-Robot Systems Under Motion and Sensing Uncertainties Using Distributed ADMM-based Trajectory Planning

Inter-robot communication enables multi-robot systems to coordinate and execute complex missions efficiently. Thus, maintaining connectivity of the communication network between robots is essential for many multi-robot systems. In this paper, we present a trajectory planner for connectivity maintenance of a multi-robot system. We first define a weighted undirected graph to represent the connectivity of the system. Unlike previous connectivity maintenance works, we explicitly account for robot motion and sensing uncertainties while formulating the graph edge weights. These uncertainties result in uncertain robot positions which directly affect the connectivity of the system. Next, the algebraic connectivity of the weighted undirected graph is maintained above a specified lower limit using a trajectory planner based on a distributed alternating direction method of multipliers (ADMM) framework. Here we derive an approximation for the Hessian matrices required within the ADMM optimization step to reduce the computational load. Finally, simulation results are presented to statistically validate the connectivity maintenance of our trajectory planner.

==> background.tex <==
\label{sec:background}

%~\cite{mohar1991laplacian}
\comment{Combine with next section?}
A multi-robot system can be represented as an undirected graph, where each node represents a robot and each edge represents the connection between two robots. Let $N$ be the number of nodes in the graph. The adjacency matrix $\mathcal{A}$ of the graph is defined as a $N \times N$ matrix such that $\mathcal{A}_{ij} \in [0,1]$ represents the edge weight between nodes $i$ and $j$. The degree of a node is defined as $d_i = \sum_{j=1}^{N} \mathcal{A}_{ij}$. The vector of node degrees $\mathbf{d}$ is then used to define the degree matrix $\mathcal{D}$ of the graph as $\mathcal{D} = \texttt{diag}(\mathbf{d})$. Given matrices $\mathcal{A}$ and $\mathcal{D}$ the Laplacian matrix $\mathcal{L}$ of the graph is defined as $\mathcal{L} = \mathcal{D} - \mathcal{A}$~\cite{grone1990laplacian}.

%As discussed in Section~\ref{subsec:global-connectivity}, algebraic connectivity is a commonly used indicator of the connectivity of multi-robot systems. It is defined as the second-smallest eigenvalue of $\mathbb{L}$, i.e., if $\lambda_1^\mathbb{L}~\leq~\lambda_2^\mathbb{L} \leq \dots \leq \lambda_N^\mathbb{L}$ are the eigenvalues of $\mathbb{L}$, then $\lambda_2^\mathbb{L}$ is the algebraic connectivity of the graph. An important property of algebraic connectivity is that it not only gives an indication on whether the graph is connected or not, but it also gives an indication of \textit{how} well-connected the graph is. The value of the algebraic connectivity varies from zero (if the graph is disconnected) to the number nodes in the graph (if the graph is fully connected), i.e. $0 \leq \lambda_2^{\mathbb{L}} \leq N$. Thus, $\lambda_2^\mathbb{L}$ is greater than zero if and only if there exists a (potentially multi-hop) communication path between any two robots in the system.

As discussed in Section~\ref{subsec:global-connectivity}, algebraic connectivity is a commonly used indicator of the connectivity of multi-robot systems. It is defined as the second-smallest eigenvalue of $\mathcal{L}$, i.e., if $\lambda_1^\mathcal{L}~\leq~\lambda_2^\mathcal{L} \leq \dots \leq \lambda_N^\mathcal{L}$ are the eigenvalues of $\mathbb{L}$, then $\lambda_2^\mathcal{L}$ is the algebraic connectivity of the graph. An important property of algebraic connectivity is that it not only gives an indication on whether the graph is connected or not, but it also gives an indication of \textit{how} well-connected the graph is. The value of the algebraic connectivity varies from zero (if the graph is disconnected) to the number nodes in the graph (if the graph is fully connected), i.e. $0 \leq \lambda_2^{\mathcal{L}} \leq N$. $\lambda_2^\mathcal{L}$ is greater than zero only if there exists a (potentially multi-hop) communication path between any two robots in the system.

%Fig.~\ref{fig:algebraic-connectivity} illustrates the algebraic connectivity for different configurations of a graph. Thus, $\lambda_2^\mathbb{L}$ remains greater than zero as long as there exists a (potentially multi-hop) communication path between any two robots in the system.

\iffalse
\begin{figure}[t]
  \centering
  \subfloat[$\lambda_2^\mathcal{L} = 0$]{%
        \includegraphics[width=0.3\linewidth]{images/ac_3_b.png}}
        \hfill
  \subfloat[$\lambda_2^\mathcal{L} = 0.3$]{%
        \includegraphics[width=0.3\linewidth]{images/ac_2_b.png}}
        \hfill
  \subfloat[$\lambda_2^\mathcal{L} = 6$]{%
        \includegraphics[width=0.3\linewidth]{images/ac_1_b.png}}
        \hfill
  \caption{The algebraic connectivity $\lambda_2^\mathcal{L}$ of a graph varies from zero (disconnected graph) to the number of nodes (fully-connected graph).}
  \label{fig:algebraic-connectivity}
  \vspace{-0.5cm}
\end{figure}
\fi

==> simulations_full.tex <==
\label{sec:simulations}
In this section, we evaluate our trajectory planning algorithm by simulating multiple missions for a multi-UAV system. We first describe the simulation setup which includes the UAV motion and sensing models, the cost functions representing the local tasks, the method used for generating initial trajectory guesses, and the values used for parameters within the planner. We then discuss the performance of our planner for two types of planning applications: \textit{offline} and \textit{online}. For \textit{offline} planning we focus on the convergence of the planner, whereas for \textit{online} planning we focus on the planner performance under time constraints. Additionally, for both applications we statistically validate the connectivity maintenance of our trajectory planning algorithm. All simulations in this section are performed on a \SI{2.80}{\GHz} Quad-core Intel\textsuperscript{TM} i7 machine.

\subsection{Simulation setup}
\label{subsec:sim-setup}

For each UAV in the multi-UAV system, we consider a 2-dimensional (2D) double integrator model as the motion model. The UAV state vector contains the 2D position and velocity, i.e, $\mathbf{x}_{i,t} = \begin{bmatrix} \mathbf{p}_{i,t}^\top & \dot{\mathbf{p}}_{i,t}^\top \end{bmatrix}^\top$, and the input vector is the UAV accelerations. The motion model for the UAV can be written in the form of Equation (\ref{eqn:motion-model}) as:
\begin{equation}
    \label{eqn:sim-motion-model}
    \mathbf{x}_{i,t} = 
    \begingroup
    \setlength\arraycolsep{3pt}
    \begin{bmatrix} 1 & 0 & dt & 0 \\ 0 & 1 & 0 & dt \\ 0 & 0 & 1 & 0 \\ 0 & 0 & 0 & 1 \end{bmatrix} 
    \endgroup
    \mathbf{x}_{i,t-1} + 
    \begingroup
    \setlength\arraycolsep{1pt}
    \begin{bmatrix} \frac{dt^2}{2} & 0 \\ 0 & \frac{dt^2}{2} \\ dt & 0 \\ 0 & dt \end{bmatrix}
    \endgroup
    \mathbf{u}_{i,t-1} + \mathbf{w}_{i,t},
\end{equation}
where $dt = \SI{0.2}{\second}$ is the time-step between two time instants and
\begin{equation*}
    \mathbf{w}_{i,t} \sim \mathcal{N} \left[ \mathbf{0}, \SI{0.1}{\metre^{2} \second^{-3}}%\num{0.1}
    \begingroup
    \setlength\arraycolsep{1pt}
    \begin{bmatrix} \frac{dt^3}{3} & 0 & \frac{dt^2}{2} & 0\\ 0 & \frac{dt^3}{3} & 0 & \frac{dt^2}{2} \\ \frac{dt^2}{2} & 0 & dt & 0 \\ 0 & \frac{dt^2}{2} & 0 & dt \end{bmatrix}
    \endgroup
    \right].
\end{equation*}
Additionally, we set a maximum limit of \SI{5}{\metre \per \square \second} on the magnitude of input accelerations. Note that in contrast to a majority of previous connectivity maintenance works, the above motion model does not assume that the UAV positions are instantaneously controllable. For the sensing model in Equation (\ref{eqn:measurement-model}), we consider position measurements:
\begin{equation}
    \label{eqn:sim-sensing-model}
    \mathbf{z}_{i,t} = \begin{bmatrix} 1 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 \end{bmatrix} \mathbf{x}_{i,t} + \mathbf{\nu}_{i,t},
\end{equation}
where
\begin{equation*}
    \mathbf{\nu}_{i,t} \sim \mathcal{N} \left[ \mathbf{0}, \begin{bmatrix} \SI{1}{\square\metre} & 0 \\ 0 & \SI{1}{\square\metre} \end{bmatrix} \right].
\end{equation*}
Additionally, we assume that each UAV operates at a different altitude, similar to \cite{park2019distributed}. We make this assumption in order to alleviate inter-UAV collision constraints and focus on the connectivity maintenance of the system.

As mentioned in Section \ref{subsec:trajecory-planning}, each UAV $i$ is considered to have a local task represented by a cost function $J_{i,t}$. For our simulations we consider the local task of reaching a desired position and minimizing the control input effort. Thus, we use the following cost functions:
\begin{align}
    \label{eqn:sim-cost-position}
    J_{i,T} & = ( \hat{\mathbf{x}}_{i,T} - \mathbf{x}_{i,\text{des}} )^\top W^{\mathbf{x}}_i ( \hat{\mathbf{x}}_{i,T} - \mathbf{x}_{i,\text{des}} ), \\
    \label{eqn:sim-cost-input}
    J_{i,t} & = \mathbf{u}_{i,t}^\top W^{\mathbf{u}}_i \mathbf{u}_{i,t},
\end{align}
where $\mathbf{x}_{i,\text{des}} = \begin{bmatrix} \mathbf{p}_{i,\text{des}}^\top & \dot{\mathbf{p}}_{i,\text{des}}^\top \end{bmatrix}^\top$ contains the desired position $\mathbf{p}_{i,\text{des}}$ and desired velocity $\dot{\mathbf{p}}_{i,\text{des}}$ for the UAV, and $W^{\mathbf{x}}_i$ and $W^{\mathbf{u}}_i$ are used to set the importance of the different costs. For our simulations we set $\dot{\mathbf{p}}_{i,\text{des}} = \mathbf{0}$.

We specify an initial position $\mathbf{p}_{i,\text{init}}$ for each UAV $i$ and set their initial velocities to be zeros, i.e., the initial state vector is $\mathbf{x}_{i,\text{init}} = \begin{bmatrix} \mathbf{p}_{i,\text{init}}^\top & \mathbf{0}^\top \end{bmatrix}^\top$. The initial state estimation covariance $\Sigma_{i,\text{init}}$ is set as:
\begin{equation}
    \label{eqn:sim-init-state-est-cov}
    \begingroup
    \setlength\arraycolsep{1pt}
    \Sigma_{i,\text{init}} = \begin{bmatrix} \SI{0.1}{\metre^2} & 0 & 0 & 0 \\ 0 & \SI{0.1}{\metre^2} & 0 & 0 \\ 0 & 0 & \SI{0.001}{\metre^2\second^{-2}} & 0 \\ 0 & 0 & 0 & \SI{0.001}{\metre^2\second^{-2}} \end{bmatrix}.
    \endgroup
\end{equation}

For our simulations, we consider the system to be comprised of two types of UAVs: \textit{primary} and \textit{bridge}. The local task for \textit{primary} UAVs includes both reaching the desired position and minimizing control input effort, thus, we set:
\begin{equation*}
    W^{\mathbf{x}}_i = \begin{bmatrix} 1 & 0 & 0 & 0\\ 0 & 1 & 0 & 0\\ 0 & 0 & 100 & 0\\ 0 & 0 & 0 & 100 \end{bmatrix}, \ \ W^{\mathbf{u}}_i = \begin{bmatrix} 0.01 & 0 \\ 0 & 0.01 \end{bmatrix},
\end{equation*}
for each UAV $i$ that is a \textit{primary} UAV. On the other hand, \textit{bridge} UAVs are not assigned a desired position and hence focus on arranging themselves in order to maintain connectivity within the system. Thus for each UAV $i$ that is a \textit{bridge} UAV, we set:
\begin{equation*}
    W^{\mathbf{x}}_i = \begin{bmatrix} 0 & 0 & 0 & 0\\ 0 & 0 & 0 & 0\\ 0 & 0 & 100 & 0\\ 0 & 0 & 0 & 100 \end{bmatrix}, \ \ W^{\mathbf{u}}_i = \begin{bmatrix} 0.01 & 0 \\ 0 & 0.01 \end{bmatrix}.
\end{equation*}

For the initial trajectory guess, we require a computationally inexpensive method of generating a trajectory based on the local tasks for each UAV. For example, sampling-based planners such as rapidly-exploring random trees (RRTs) can be used in order to quickly plan trajectories around obstacles \cite{van2012motion,goretkin2013optimal}; in a multiple target tracking application, each UAV can be randomly assigned to track a separate target \cite{park2019distributed}. In our algorithm, we use a linear-quadratic-regulator (LQR) to obtain an initial trajectory guess for each \textit{primary} UAV $i$ from $\mathbf{x}_{i,\text{init}}$ to $\mathbf{x}_{i,\text{des}}$. For \textit{bridge} UAVs, we simply set the initial trajectory guess to be hovering at the initial position. If our metric $\underline{\lambda}_2^{\mathbb{L}_t}$ is not maintained above $\epsilon$ for the resulting trajectory guess of the multi-UAV system, we consider new desired states (only for the initial trajectory guess and not for the rest of the planner) midway between $\mathbf{x}_{i,\text{init}}$ and the $\mathbf{x}_{i,\text{des}}$ for all \textit{primary} UAVs and repeat the process.

We consider a communication range of $\Delta = \SI{40}{\metre}$ and set the parameter $\Delta_0 = \SI{35}{\metre}$ in Equation (\ref{eqn:conservative-edge-weight}). For the connectivity maintenance requirement in Equation (\ref{eqn:connectivity-maintenance}), we set the lower algebraic connectivity limit $\epsilon = \num{0.1}$ and the corresponding probability value $\delta = \num{0.003}$ to reflect a $3\sigma$ confidence level. We set $T = \num{250}$, which results in a planning time horizon of \SI{50}{\second}. In Equation (\ref{eqn:connectivity-cost}), we set the parameter for the magnitude of the connectivity cost as $k_c = \num{0.001}$. We set $\eta = \num{2}$ for the number of elements in subsets $\mathcal{V}$ obtained in the trajectory planner. Finally, for the line search algorithm used to update the ADMM consensus variable in Equation (\ref{eqn:admm-line-search}), we set $\gamma = \num{0.8}$.

\subsection{Offline planning}
\label{subsec:offline-planning}

For \textit{offline} planning applications, we simulate two missions for a system with five UAVs. For the first \textit{offline} mission we consider all five UAVs to be \textit{primary} UAVs. Here we set the desired positions for the UAVs at a sufficient relative distance such that the system connectivity would not be maintained if each UAV reaches its desired position. Thus, the planner attempts to find trajectories such that each UAV reaches as close as possible to its desired position while still satisfying the connectivity requirement from Equation (\ref{eqn:connectivity-maintenance}). Fig. \ref{fig:mission-1} shows the results for the first \textit{offline} mission.
\iffalse
Since all UAVs are \textit{primary}, each is tasked with reaching a desired position $\mathbf{p}_{i,\text{des}}$. We set the desired final velocity $\dot{\mathbf{p}}_{i,\text{des}}$ to be zero. Thus, the desired state vector is $\mathbf{x}_{i,\text{des}}~=~\begin{bmatrix} \mathbf{p}_{i,\text{des}}^\top & \mathbf{0}^\top \end{bmatrix}^\top$.\fi

Figs. \ref{fig:mission-1}(a)-(d) show the process of convergence of our trajectory planning algorithm. The planner begins by generating an initial trajectory guess using the LQR-based method discussed in Section \ref{subsec:sim-setup}. Fig. \ref{fig:mission-1}(d) shows the final planned trajectories obtained after the convergence-based stopping criteria has been satisfied. Additionally, we simulate $1000$ trajectory rollouts for the multi-UAV system where each UAV tracks the planned trajectory using LQR. The simulated rollouts are later used to statistically validate the system connectivity. In Fig. \ref{fig:mission-1}(e), we show the convergence of the cost in the transformed optimization problem from Equation (\ref{eqn:transformed-opt-problem}). 
%Note that since the belief-space iLQG computes a locally optimal trajectory for the non-convex cost function in Equation (\ref{eqn:admm-opt}), the output from our planning algorithm is not globally optimal.

Fig. \ref{fig:mission-1}(f) shows the connectivity maintenance of the system along the planned trajectories. Given that we incorporated the connectivity cost function (Equation (\ref{eqn:connectivity-cost})) in the transformed optimization problem (Equation (\ref{eqn:transformed-opt-problem})), the planned trajectories maintain our metric  $\underline{\lambda}_2^{\mathbb{L}}$ above the lower limit $\epsilon$. As discussed in Section \ref{sec:connectivity-metric}, maintaining $\underline{\lambda}_2^{\mathbb{L}} > \epsilon$ results in satisfying the connectivity maintenance requirement described in Equation (\ref{eqn:connectivity-maintenance}). In order to statistically validate that this requirement is satisfied, we compare the algebraic connectivity ${\lambda}_2^{\mathbb{L}}$ of the $1000$ simulated rollouts against the lower limit $\epsilon$ in Fig. \ref{fig:mission-1}(f). Only one (colored red) of the $1000$ rollouts results in a ${\lambda}_2^{\mathbb{L}}$ below $\epsilon$. Given that we set the probability value $\delta = \num{0.997}$, this statistically validates the connectivity maintenance requirement from Equation (\ref{eqn:connectivity-maintenance}).

\begin{figure*}[t]
  \centering
  \subfloat{%
        \includegraphics[width=0.5\linewidth,trim={0cm 0cm 0cm 0},clip]{images/m1_paths_leg.png}} \addtocounter{subfigure}{-1}
        \hfill \\
        \vspace{-0.2cm}
  \subfloat[]{%
        \includegraphics[width=0.24\linewidth,trim={4cm 0 5cm 0},clip]{images/m1_paths_iter0.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.24\linewidth,trim={4cm 0 5cm 0},clip]{images/m1_paths_iter2.png}}
        \hfill
  \subfloat[]{%
       \includegraphics[width=0.24\linewidth,trim={4cm 0 5cm 0},clip]{images/m1_paths_iter5.png}}
       \hfill
  \subfloat[]{%
        \includegraphics[width=0.24\linewidth,trim={4cm 0 5cm 0},clip]{images/m1_paths_final.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.35\linewidth,trim={1.5cm 0 3cm 0},clip]{images/m1_cost.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.55\linewidth,trim={3cm 0 4cm 0},clip]{images/m1_algebraic_connectivity.png}}
        \hfill
  \caption{Trajectory planning and connectivity maintenance for \textit{offline} mission with five \textit{primary} UAVs. (a)-(d) Convergence of the planned trajectories. (e) Convergence of the cost in the transformed optimization problem (Equation (\ref{eqn:transformed-opt-problem})). (f) Statistical validation of connectivity maintenance throughout the mission. Only one (red) of the $1000$ trajectory rollouts results in algebraic connectivity ${\lambda}_2^{\mathbb{L}}$ less than the lower limit $\epsilon$.}
  \label{fig:mission-1}
\end{figure*}

For the second \textit{offline} mission, we consider the multi-UAV system to consist of three \textit{primary} UAVs and two \textit{bridge} UAVs. Each \textit{primary} UAV is tasked with reaching a desired position, whereas the \textit{bridge} UAVs are not assigned any desired positions. Fig. \ref{fig:mission-2} shows the results for the second \textit{offline} mission. The convergence of our planning algorithm is shown in Figs. \ref{fig:mission-2}(a)-(d). For the initial trajectory guess, we use the LQR-based method for the \textit{primary} UAVs, whereas for the \textit{bridge} UAVs we set them to be hovering at their initial positions. We observe that the final planned trajectories for the \textit{primary} UAVs reach their desired positions, while the \textit{bridge} UAVs arrange themselves in order to maintain connectivity within the system. Similar to the first \textit{offline} mission, we simulate $1000$ trajectory rollouts where each UAV uses LQR to track the planned trajectories. Fig. \ref{fig:mission-2}(e) shows the convergence of the cost in the transformed optimization problem from Equation (\ref{eqn:transformed-opt-problem}).

In Fig. \ref{fig:mission-2}(f) we show the connectivity maintenance of the system. The planned trajectories maintain our metric $\underline{\lambda}_2^{\mathbb{L}}$ above the lower limit $\epsilon$. For only two (colored magenta) of the $1000$ rollouts the algebraic connectivity ${\lambda}_2^{\mathbb{L}}$ drops below our metric $\underline{\lambda}_2^{\mathbb{L}}$, whereas none drop below the lower limit $\epsilon$. This statistically validates that the connectivity maintenance requirement from Equation (\ref{eqn:connectivity-maintenance}) is satisfied.

\begin{figure*}[]
  \centering
  \subfloat{%
        \includegraphics[width=0.7\linewidth,trim={0cm 0cm 0cm 0},clip]{images/m2_paths_leg.png}} \addtocounter{subfigure}{-1}
        \hfill \\
        \vspace{-0.3cm}
  \subfloat[]{%
        \includegraphics[width=0.24\linewidth,trim={4cm 0 5cm 0},clip]{images/m2_paths_iter0.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.24\linewidth,trim={4cm 0 5cm 0},clip]{images/m2_paths_iter2.png}}
        \hfill
  \subfloat[]{%
       \includegraphics[width=0.24\linewidth,trim={4cm 0 5cm 0},clip]{images/m2_paths_iter5.png}}
       \hfill
  \subfloat[]{%
        \includegraphics[width=0.24\linewidth,trim={4cm 0 5cm 0},clip]{images/m2_paths_final.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.35\linewidth,trim={1.5cm 0 3cm 0},clip]{images/m2_cost.png}}
        \hfill
   \subfloat[]{%
        \includegraphics[width=0.55\linewidth,trim={3cm 0 4cm 0},clip]{images/m2_algebraic_connectivity.png}}
        \hfill
  \caption{Trajectory planning and connectivity maintenance for \textit{offline} mission with three \textit{primary} UAVs and two \textit{bridge} UAVs. (a)-(d) Convergence of the planned trajectories. (e) Convergence of the cost in the transformed optimization problem (Equation (\ref{eqn:transformed-opt-problem})). (f) Statistical validation of connectivity maintenance throughout the mission. Only two (magenta) of the $1000$ trajectory rollouts results in algebraic connectivity ${\lambda}_2^{\mathbb{L}}$ less than our metric $\underline{\lambda}_2^{\mathbb{L}}$, whereas none drop below the lower limit $\epsilon$.}
  \label{fig:mission-2}
\end{figure*}

\subsection{Online planning}
\label{subsec:online-planning}

For \textit{online} planning applications, we evaluate our planning algorithm on two missions under time constraints. We consider an \textit{online} mission to be comprised of multiple segments and allot a maximum planning time for each segment. This resembles applications such as exploration, coverage, or formation control, where only a limited amount of computation time is available for planning trajectories while the remaining time is required for other purposes such as analyzing sensor data or decision making. Given that we consider multiple segments in the mission, we plan the trajectories for the upcoming mission segment while executing the planned trajectories for the current mission segment. Fig. \ref{fig:online-mission-timeline} shows the order of planning and trajectory execution for an \textit{online} mission. We set a maximum planning time of \SI{25}{\second} and a trajectory duration of \SI{50}{\second} for each mission segment. Additionally, since our planner potentially requires multi-hop communication, we account for a delay of \SI{0.2}{\second} in each ADMM iteration of our planning algorithm (Algorithm \ref{alg:admm}).

For the first \textit{online} mission, we consider a multi-UAV system with three \textit{primary} and two \textit{bridge} UAVs. The \textit{primary} UAVs are tasked with reaching different desired positions in each segment. Fig. \ref{fig:mission-3} shows the results for the first \textit{online} mission. Here, the desired positions for the first segment are selected similar to the desired positions in the second \textit{offline} mission (Fig. \ref{fig:mission-2}). Note that due to a limited planning time, the planned trajectories for the first segment do not converge to the desired positions for all UAVs. However, as discussed in Section \ref{subsec:admm-setup}, the output from our trajectory planning algorithm always satisfies the connectivity maintenance requirement from Equation (\ref{eqn:connectivity-maintenance}). Fig. \ref{fig:mission-3}(a) shows the planned trajectories for the first segment along with $1000$ trajectory rollouts of the system. The final UAV positions from the first segment are then used as initial positions while planning for the second segment. Figs. \ref{fig:mission-3}(b) and \ref{fig:mission-3}(c) show the planned trajectories and rollouts for the second and third segments. The convergence of the cost from Equation (\ref{eqn:transformed-opt-problem}) for the first three segments is shown in Figs. \ref{fig:mission-3}(d)-(f). Note that the order of trajectory planning is as shown in Fig. \ref{fig:online-mission-timeline}. Fig \ref{fig:mission-3}(g) shows the connectivity maintenance results for the complete mission. Our connectivity metric $\underline{\lambda}_2^{\mathbb{L}}$ is maintained above the lower limit $\epsilon$ throughout the mission. From the $1000$ simulated rollouts, we observe that the algebraic connectivity ${\lambda}_2^{\mathbb{L}}$ for only two (colored magenta) rollouts drop below our metric $\underline{\lambda}_2^{\mathbb{L}}$, while none drop below the limit $\epsilon$.

For the second \textit{online} mission, in order to evaluate our planner for a larger multi-UAV system, we consider ten UAVs: six \textit{primary} and four \textit{bridge}. Additionally, as shown in Fig. \ref{fig:mission-4} we consider the mission to consist of six segments in order to show the planning results for a variety of configurations of the desired UAV positions. Figs. \ref{fig:mission-4}(a)-(f) show the planned trajectories for the six segments and Figs. \ref{fig:mission-4}(g)-(l) show the convergence of the corresponding costs. In Fig. \ref{fig:mission-4}, we show the connectivity maintenance throughout the mission. Similar to the first \textit{online} mission, our metric $\underline{\lambda}_2^{\mathbb{L}}$ is maintained above the lower limit $\epsilon$. The algebraic connectivity of only one (colored magenta) of the $1000$ simulated rollouts drops below $\underline{\lambda}_2^{\mathbb{L}}$, while none drop below $\epsilon$. Thus, the connectivity maintenance requirement from Equation (\ref{eqn:connectivity-maintenance}) is satisfied for both \textit{online} missions.

\begin{figure}[]
    \centering
    \includegraphics[width=\linewidth]{images/online_mission_timeline_alt.png}
    \caption{Order of trajectory planning (orange) and execution (blue) for \textit{online} planning applications. We allot a maximum planning time for each segment since the remaining time (yellow) could be required for other purposes such as analyzing sensor data or decision making.}
    \label{fig:online-mission-timeline}
\end{figure}

\begin{figure*}[]
  \centering
  \subfloat{%
        \includegraphics[width=0.7\linewidth,trim={0cm 0cm 0cm 0},clip]{images/m3_paths_leg.png}} \addtocounter{subfigure}{-1}
        \hfill \\
        \vspace{-0.3cm}
  \subfloat[]{%
        \includegraphics[width=0.3\linewidth,trim={4cm 0 4cm 0},clip]{images/m3_paths_1.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.3\linewidth,trim={4cm 0 4cm 0},clip]{images/m3_paths_2.png}}
        \hfill
  \subfloat[]{%
       \includegraphics[width=0.3\linewidth,trim={4cm 0 4cm 0},clip]{images/m3_paths_3.png}}
       \hfill %\\ 
        %\hspace{2cm}
  \subfloat[]{%
        \includegraphics[width=0.2\linewidth,trim={0 0 1cm 0},clip]{images/m3_cost_1.png}}
        %\hfill
        \hspace{1cm}
  \subfloat[]{%
        \includegraphics[width=0.2\linewidth,trim={0 0 1cm 0},clip]{images/m3_cost_2.png}}
        %\hfill
        \hspace{1cm}
  \subfloat[]{%
        \includegraphics[width=0.2\linewidth,trim={0 0 1cm 0},clip]{images/m3_cost_3.png}}
        %\hspace{3cm}
        \hfill
    \subfloat[]{%
        \includegraphics[width=\linewidth]{images/m3_algebraic_connectivity.png}}
        \hfill
  \caption{Trajectory planning and connectivity maintenance for \textit{online} mission with three \textit{primary} and two \textit{bridge} UAVs. (a)-(c) The final planned trajectories and rollouts for each segment of the mission. (d)-(f) Convergence of the cost in the transformed optimization problem for a maximum planning time of \SI{25}{\second}. (g) Statistical validation of connectivity maintenance throughout the mission. Only two (magenta) of the $1000$ trajectory rollouts results in algebraic connectivity ${\lambda}_2^{\mathbb{L}}$ less than our metric $\underline{\lambda}_2^{\mathbb{L}}$, whereas none drop below the lower limit $\epsilon$.}
  \label{fig:mission-3}
\end{figure*}

\begin{figure*}[]
  \centering
  \subfloat{%
        \includegraphics[width=0.7\linewidth,trim={0cm 0cm 0cm 0},clip]{images/m4_paths_leg.png}} \addtocounter{subfigure}{-1}
        \hfill \\
        \vspace{-0.35cm}
  \subfloat[]{%
        \includegraphics[width=0.3\linewidth,trim={4cm 0 4cm 0},clip]{images/m4_paths_1.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.3\linewidth,trim={4cm 0 4cm 0},clip]{images/m4_paths_2.png}}
        \hfill
  \subfloat[]{%
       \includegraphics[width=0.3\linewidth,trim={4cm 0 4cm 0},clip]{images/m4_paths_3.png}}
       \hfill
       \vspace{-0.35cm}
  \subfloat[]{%
        \includegraphics[width=0.3\linewidth,trim={4cm 0 4cm 0},clip]{images/m4_paths_4.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.3\linewidth,trim={4cm 0 4cm 0},clip]{images/m4_paths_5.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.3\linewidth,trim={4cm 0 4cm 0},clip]{images/m4_paths_6.png}}
        \hfill
        \vspace{-0.1cm}
  \subfloat[]{%
        \includegraphics[width=0.16\linewidth,trim={0 0 1cm 0},clip]{images/m4_cost_1.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.16\linewidth,trim={0 0 1cm 0},clip]{images/m4_cost_2.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.16\linewidth,trim={0 0 1cm 0},clip]{images/m4_cost_3.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.16\linewidth,trim={0 0 1cm 0},clip]{images/m4_cost_4.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.16\linewidth,trim={0 0 1cm 0},clip]{images/m4_cost_5.png}}
        \hfill
  \subfloat[]{%
        \includegraphics[width=0.16\linewidth,trim={0 0 1cm 0},clip]{images/m4_cost_6.png}}
        \hfill
        \vspace{-0.1cm}
  \subfloat[]{%
        \includegraphics[width=\linewidth]{images/m4_algebraic_connectivity.png}}
        \hfill
        \vspace{-0.2cm}
  \caption{Trajectory planning and connectivity maintenance for \textit{online} mission with six \textit{primary} and four \textit{bridge} UAVs. (a)-(f) The final planned trajectories and rollouts for each segment of the mission. (g)-(l) Convergence of the cost in the transformed optimization problem for a maximum planning time of \SI{25}{\second}. (m) Statistical validation of connectivity maintenance throughout the mission. Only one (magenta) of the $1000$ trajectory rollouts results in algebraic connectivity ${\lambda}_2^{\mathbb{L}}$ less than our metric $\underline{\lambda}_2^{\mathbb{L}}$, whereas none drop below the lower limit $\epsilon$.}
  \label{fig:mission-4}
\end{figure*}
